SafeBPF: Hardware-assisted Defense-in-depth for eBPF Kernel Extensions

The eBPF framework enables execution of user-provided code in the Linux kernel. In the last few years, a large ecosystem of cloud services has leveraged eBPF to enhance container security, system observability, and network management. Meanwhile, incessant discoveries of memory safety vulnerabilities have left the systems community with no choice but to disallow unprivileged eBPF programs, which unfortunately limits eBPF use to only privileged users. To improve run-time safety of the framework, we introduce SafeBPF, a general design that isolates eBPF programs from the rest of the kernel to prevent memory safety vulnerabilities from being exploited. We present a pure software implementation using a Software-based Fault Isolation (SFI) approach and a hardware-assisted implementation that leverages ARM's Memory Tagging Extension (MTE). We show that SafeBPF incurs up to 4% overhead on macrobenchmarks while achieving desired security properties.

==> analogs.tex <==
\input{listing/instruction-analog.tex}

\change{\autoref{fig:insa} shows ...}

==> design.tex <==
\system enforces memory safety at runtime. 
In addition to the static checks performed by the \ebpf verifier, \system ensures that all accesses to \ebpf data (\eg \ebpf maps, \ebpf stack and \ebpf context) are always bounded at runtime.
We instrument the x86 and ARM JIT compilers to rewrite \ebpf binaries.
\system inserts dynamic checks to each load and store instructions in an \ebpf program, assuring both confidentiality and integrity of kernel memory.
The instrumentation is fully-automated and requires no manual annotation, which complies with our threat model that \ebpf users are malicious and hence user annotations cannot be trusted.

We design \system to be \emph{minimally invasive}, reusing the existing eBPF pipeline and extending only what is necessary. 
Specifically, SandBPF adds binary rewriting only at the end of the JIT compilation, as shown in Figure X. 
Since \system performs rewriting on the final output of \ebpf's JIT compilation, it does not rely on the correctness of the JIT compiler or the verifier, which have both been found buggy.
Furthermore, this design allows experienced users to develop eBPF programs like they normally do, while new users can rely on existing eBPF documentation.

In this section, we describe \system high-level design and primitives.
In \autoref{sec:implementation}, we will discuss enforcement mechanisms and in \autoref{sec:evaluation} compare their performances.

\noindgras{\circled{1} Something.} blablabla.

\noindgras{\circled{2} Something else.} blablabla.


\subsection{Sandbox Management}
\label{sec:sandbox-management}

\system reserves one memory page in each processor core for storing \system's metadata and the data of a sandboxed \ebpf program, as illustrated in~\autoref{fig:design}.
While the content in the \emph{metadata} partition depends on the isolation techniques in~\autoref{sec:implementation:checks}, the \emph{sandbox} partition will always contain the stack and context of an \ebpf program. 
\ebpf does not support dynamic memory allocation as the \ebpf verifier cannot resolve dynamically-allocated memory at compile time.
With the addition of runtime checks, \system adds support for dynamic memory allocation in the sandbox partition, with the heap information stored in the metadata partition.

Upon the invocation of an \ebpf program, the context in the sandbox partition is initialized.
The context is the input to an \ebpf program, which varies depending on the \ebpf program type.
For example, the context of a socket filter program is \texttt{\_\_sk\_buff}, a mirror of the \texttt{sk\_buff} structure.
When an \ebpf program accesses the context (\texttt{\_\_sk\_buff}), all load/store instructions to the context are transparently transformed into accesses to the actual kernel data structure (\texttt{sk\_buff}) at compile time.
Instead, \system copies only the fields specified in the context to the sandbox partition, disallowing access to the kernel data structure. 
At the end of JIT compilation, \system rewrites the \ebpf program to use the stack and context in the sandbox partition at runtime.
\system cleans up the sandbox upon \ebpf program termination in preparation for the next \ebpf program invocation.

We disable interrupt and preemption during the execution of an eBPF program, so each core runs only one eBPF program at a time.
Preemption was disabled for all \ebpf programs until Linux v5.11~\cite{preemption-misc}.
As more features are introduced into \ebpf, preemption was turned off to allow \ebpf programs to, for example, call blocking functions or share data via per-CPU maps.
In \system, we re-disable preemption and require that \ebpf programs cannot sleep during execution.
Therefore, \system does not support sleepable \ebpf programs, such as \texttt{BPF\_PROG\_TYPE\_LSM}, \texttt{BPF\_PROG\_TYPE\_KPROBE}, \texttt{BPF\_PROG\_TYPE\_STRUCT\_OPS}, and \texttt{BPF\_PROG\_TYPE\_TRACING}.


\subsection{Handling \ebpf Maps}
\ebpf maps are key/value stores that can be shared between multiple \ebpf programs, and between \ebpf programs and user space applications. 
To ensure spatial memory safety, \system emits runtime checks on all instructions that access \ebpf map values, preventing \ebpf programs from accessing kernel memory outside of the map.
In particular, \system ensures that only the map value region is accessible, as seen in~\autoref{fig:design}.
The metadata of an \ebpf map (\eg reference count and synchronization primitives) cannot be directly accessed by any \ebpf programs.
While \system currently supports only \texttt{BPF\_MAP\_TYPE\_ARRAY}, the implementation discussed in~\autoref{sec:implementation} is also applicable to other \ebpf map types.
We further discuss this in~\autoref{sec:discussion}.




==> figure/costbreakdown-x86.tex <==
\pgfplotstableread{
	Label prog mng mem tramp
	XDP 4859.907619 736.562105 173.6002732 32.60799579
	{Socket Filter}  1632.1 349.0639471 190.1571767 83.88
	Katran 0 0 0 0
}\breakdowndata

\begin{figure}[t]
	\centering
	\begin{tikzpicture}
		\begin{axis}[
			ybar stacked,
			ymin=0,
			ymax=6000,
			xtick=data,
			legend style={at={(0.5,-0.1)},anchor=north},
			reverse legend=true,
			xticklabels from table={\breakdowndata}{Label},
			ylabel={nanoseconds}
			]
			\addplot
			table [y=prog, meta=Label, x expr=\coordindex]
			{\breakdowndata};
			\addlegendentry{eBPF Program}
			\addplot
			table [y=mng, meta=Label, x expr=\coordindex]
			{\breakdowndata};
			\addlegendentry{Context Synchronization}
			\addplot
			table [y=mem, meta=Label, x expr=\coordindex]
			{\breakdowndata};
			\addlegendentry{Sandbox Management}
			\addplot[fill=orange!60,point meta=y]
			table [y=tramp, meta=Label, x expr=\coordindex]
			{\breakdowndata};
			\addlegendentry{Access Checks}
		\end{axis}
	\end{tikzpicture}
	\caption{Breakdown of the overhead introduced by \system 
		on our three example \ebpf programs.}
	\label{fig:cost-x86}
\end{figure}

==> listing/instruction-analog.tex <==
\begin{figure}[t]
	\centering
	\noindent
	\begin{lstlisting}[language={[ARM]Assembler},gobble=5,numbers=left,frame=tb]
	; Simple store operation
	str x1, <address>
	
	; Instruction analogs for store 
	ldr x1, <tag address>
	str x1, <address>
	\end{lstlisting}
	\caption{Instruction analog example for \texttt{str} instruction.}
	\label{fig:insa}
\end{figure}

==> sundburst.tex <==
\newlength{\layerwd}
\newcounter{outermost}


\NewDocumentEnvironment{onion}{sm}{%
	\begin{tikzpicture}
		\setlength{\layerwd}{#2}%
		\setcounter{outermost}{0}
	}{%
		\foreach \A in {0,...,\theoutermost}{\draw[thick] (0,0) circle (\A*\layerwd+\layerwd);
		\node[fill=white,align=left] at (0,0) {57};}
	\end{tikzpicture}
}

\NewDocumentCommand{\annulus}{sO{lightgray}mmmo}{%
	\filldraw[thick,fill=#2] (#4:#3*\layerwd) %
	arc [radius=#3*\layerwd, start angle=#4, delta angle=#5-#4] %
	-- (#5:#3*\layerwd+\layerwd) %
	arc [radius=#3*\layerwd+\layerwd, start angle=#5, delta angle=#4-#5] %
	-- cycle; %
	\pgfmathsetmacro{\tmp}{(#5-#4)/2 +#4} %
	\IfNoValueF{#6}{%
		\IfBooleanTF{#1}
		{%
			\begingroup
			\pgfmathsetmacro{\rpTF}{ifthenelse(\tmp>180,"false","true")}
			\def\\{\space} %
			\path[rotate=\tmp-180,postaction={
				decorate,
				decoration={
					text along path,
					raise=-3pt,
					text align={align=center},
					reverse path=\rpTF,
					text=#6
				}
			}] (0,0) circle (#3*\layerwd+0.5*\layerwd);
			\endgroup
		}%
		{%
			\pgfmathsetmacro{\rpTF}{ifthenelse(\tmp>180,\tmp+90,\tmp-90)}
			\node[inner sep=0pt, %
			text width=#3*\layerwd*3+\layerwd,
			align=center,
			rotate=\rpTF,
			font=\footnotesize] at (\tmp:#3*\layerwd+0.5*\layerwd)
			{#6};
		}%
	}%
	\ifnum\theoutermost<#3\setcounter{outermost}{#3}\fi
}

==> x86.tex <==
\notetp{Describe the machine we used to run the experiment + Linux version \etc}

\subsection{Microbenchmark}

\input{figure/costbreakdown-x86}

\notetp{Discuss any difference with the ARM approach and explain it.}

\subsection{Macrobenchmark}

\notetp{Discuss any difference with the ARM approach and explain it.}
